Self-Attention and Ingredient-Attention Based Model for Recipe Retrieval from Image Queries

Direct computer vision based-nutrient content estimation is a demanding task, due to deformation and occlusions of ingredients, as well as high intra-class and low inter-class variability between meal classes. In order to tackle these issues, we propose a system for recipe retrieval from images. The recipe information can subsequently be used to estimate the nutrient content of the meal. In this study, we utilize the multi-modal Recipe1M dataset, which contains over 1 million recipes accompanied by over 13 million images. The proposed model can operate as a first step in an automatic pipeline for the estimation of nutrition content by supporting hints related to ingredient and instruction. Through self-attention, our model can directly process raw recipe text, making the upstream instruction sentence embedding process redundant and thus reducing training time, while providing desirable retrieval results. Furthermore, we propose the use of an ingredient attention mechanism, in order to gain insight into which instructions, parts of instructions or single instruction words are of importance for processing a single ingredient within a certain recipe. Attention-based recipe text encoding contributes to solving the issue of high intra-class/low inter-class variability by focusing on preparation steps specific to the meal. The experimental results demonstrate the potential of such a system for recipe retrieval from images. A comparison with respect to two baseline methods is also presented.

==> data-examples.tex <==
\begin{table*}
\begin{tabular}{|c|c|c|}
 \hline
 \large\textbf{Meal Image} & \large\textbf{Ingredients} & \large\textbf{Instructions} \\ [0.3ex] 
 \hline
  \begin{minipage}{.25\textwidth}
      \includegraphics[width=\linewidth, height=30mm]{images/chicken}
  \end{minipage} 
  & 
  \begin{tabular}{l}
  \small{1. chicken} \\
  \small{2. garlic} \\
  \small{3. butter} \\
  \small{4. lemon} \\
  \small{5. rosemary}\\
  \small{6. basil}\\
  \small{7. thyme}\\
  \small{8. salt and pepper}
  \end{tabular}
  & 
  \begin{tabular}{l}
  \small{1. Preheat oven to 370F.}\\
  \small{2. Rub salt and pepper to the chicken and set aside for around 10 mins.} \\
  \small{3. rub half of the butter to the chicken.} \\
  \small{4. Mince 1 whole garlic and rub on the chicken.}\\
  \small{5. Rub chicken with Herbs.}\\
  \small{6. Stuff chicken with lemon, butter, 1 whole garlic, salt, pepper and herbs.}\\
  \small{7. Put chicken in oven covered with foil for 45 mins.}\\
  \small{8. Remove cover and cook for another 45 mins at 400F}
  \end{tabular} \\ 
   \hline
   \begin{minipage}{.25\textwidth}
       \includegraphics[width=\linewidth,  height=33mm]{images/cake}
   \end{minipage}
   & 
   \begin{tabular}{l}
   \small{1. ladyfingers} \\
   \small{2. cream cheese}\\
   \small{3. lemon juice} \\
   \small{4. lemon jelly powder} \\
   \small{5. boiling water}\\
   \small{6. ice cubes}\\
   \small{7. Cool Whip Topping}\\
   \small{8. fresh raspberries}\\
   \small{9. jelly powder}
   \end{tabular} 
   & 
   \begin{tabular}{l}
   \small{1. Grease 9 inch (23 cm) springform pan.} \\
   \small{2. Place lady fingers around inside rim and set aside} \\
   \small{3. Beat cream cheese in large bowl of electric mixer.} \\
   \small{4. Add lemon juice and rind, beating on low speed until blended.} \\
   \small{5. Dissolve lemon jelly powder in boiling water.}\\
   \small{6. Add ice cubes, stirring until slightly thickened.}\\
   \small{7. Add lemon jelly slowly to cream cheese mixture while beating.}\\
   \small{8. Increase speed and beat just until well blended.}\\
   \small{9. etc. ...}
   \end{tabular} \\  
   \hline
   \begin{minipage}{.25\textwidth}
       \includegraphics[width=23mm,  height=30mm]{images/drink}
   \end{minipage} 
   & 
   \begin{tabular}{l}
   \small{1. strawberries} \\
   \small{2. pineapple} \\
   \small{3. non-dairy coffee creamer} \\
   \small{4. orange juice}
   \end{tabular} 
   & 
   \begin{tabular}{l}
   \small{1. In blender add strawberries, pineapple, non-dairy}\\
   \small{\:\:\:creamer and orange juice and blend until smooth.} \\
   \small{2. Poor into frosted glass and enjoy!}
   \end{tabular}  \\
 \hline
\end{tabular}
\caption{Recipe samples from the Recipe1M Dataset}
\label{table:recipes}
\end{table*}

==> retrievals.tex <==
\begin{table*}
\begin{tabular}{|c|c|c|}
 \hline
 \large\textbf{Sample 1} & \large\textbf{Sample 2} & \large\textbf{Sample 3}  \\ 
 \hline
 
 \begin{tabular}{c|c|c}
    \multicolumn{2}{ c| }{meal image} & ingredients\\ 
    \hline  
    \rotatebox[origin=c]{90}{Query}
    &
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=10mm, height=16mm]{retrieval_images/good_query}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. marinade} \\
    \small{2. whole chicken} \\
    \small{3. salt} \\
    \small{4. garlic powder} \\
    \small{5. onion powder}
    \end{tabular}\\ 
    
    \hline
    \hline
    
    \rotatebox[origin=c]{90}{Top 1 retrieval}
    &
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=10mm, height=16mm]{retrieval_images/good_top1}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \textit{\small{1. whole chicken}} \\
    \small{2. ground black pepper} \\
    \textit{\small{3. onion powder}} \\
    \small{4. cayenne pepper} \\
    \textit{\small{5. garlic powder}}\\
    \small{6. garlic cloves}\\
    \small{7. dried thyme}\\
    \small{8. chicken}\\
    \small{9. butter}
    \end{tabular}\\ 
    
     \hline
    
    \rotatebox[origin=c]{90}{Top 2 retrieval}
    &
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/good_top2}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. chicken drumsticks} \\
    \small{2. sea salt} \\
    \small{3. ground black pepper} \\
    \textit{\small{4. garlic powder }} \\
    \small{5. onion powder}\\
    \small{6. dried oregano}\\
    \small{7. dried chipotle powder}\\
    \small{8. ground cumin}\\
    \small{9. coconut sugar crystals}
    \end{tabular}\\ 
    
     \hline
    
    \rotatebox[origin=c]{90}{Top 3 retrieval}
    &
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/good_top3}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \textit{\small{1. whole chicken}} \\
    \small{2. lime} \\
    \small{3. paprika} \\
    \small{4. cumin} \\
    \small{5. salt and pepper}
    \end{tabular}\\ 
  \end{tabular} 
  
  
  &
  
  
  \begin{tabular}{c|c}
    meal image & ingredients\\ 
    \hline  
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/medium_query}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. cooked chicken breasts} \\
    \small{2. grapes} \\
    \small{3. feta cheese} \\
    \small{4. celery} \\
    \small{5. dried onion flakes}\\
    \small{6. cashews}\\
    \small{7. parsley}\\
    \small{8. salt and pepper}\\
    \small{9. mayonnaise}
    \end{tabular}\\ 
    
    \hline
    \hline
    
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/medium_top1}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \textit{\small{1. cooked chicken breasts}} \\
    \textit{\small{2. celery}} \\
    \textit{\small{3. mayonnaise}} \\
    \small{4. sour cream} \\
    \small{5. fresh rosemary}
    \end{tabular}\\ 
    
     \hline
    
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/medium_top2}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. tuna} \\
    \textit{\small{2. celery}} \\
    \small{3. sweet pickle} \\
    \textit{\small{4. mayonnaise}}
    \end{tabular}\\ 
    
     \hline
    
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/medium_top3}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. 1 can Canned tuna} \\
    \textit{\small{2. celery}} \\
    \small{3. dill} \\
    \small{4. lemon juice} \\
    \textit{\small{5. mayonnaise}}\\
    \textit{\small{8. salt and pepper}}
    \end{tabular}\\ 
  \end{tabular}
  
  
  &
  
  
  \begin{tabular}{c|c}
    meal image & ingredients\\ 
    \hline  
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/bad_query}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. water} \\
    \small{2. crabmeat} \\
    \small{3. parmesan cheese} \\
    \small{4. lemon juice} \\
    \small{5. mayonnaise}\\
    \small{6. lack pepper}
    \end{tabular}\\ 
    
    \hline
    \hline
    
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/bad_top1}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. 2 can Cream of Chicken} \\
    \small{2. 2 can Cream of mushroom} \\
    \small{3. Cooked chicken} \\
    \small{4. egg noodles} \\
    \small{5. onion}\\
    \small{6. ream cheese}\\
    \small{7. milk}\\
    \small{8. sour cream}\\
    \small{9. ranch seasoning}\\
    \small{10. cream of celery soup}
    \end{tabular}\\ 
    
     \hline
    
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/bad_top2}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. fettuccine} \\
    \small{2. cooked chicken breasts} \\
    \small{3. cream of chicken soup} \\
    \small{4. sour cream} \\
    \small{5. onions}\\
    \small{6. dried parsley}\\
    \small{7. white wine }\\
    \small{8. cheddar cheese}
    \small{9. salt}
    \end{tabular}\\ 
    
     \hline
    
    \begin{minipage}{.12\textwidth}
      \includegraphics[width=\linewidth, height=16mm]{retrieval_images/bad_top3}
    \end{minipage} 
    & 
    \setlength\extrarowheight{-3pt}
    \begin{tabular}{l}
    \small{1. chicken} \\
    \small{2. noodles} \\
    \textit{\small{3. mayonnaise}} \\
    \small{4. onions} \\
    \small{5. salt}\\
    \small{6. cream of mushroom soup}\\
    \small{7. milk}\\
    \small{8. cheddar cheese}
    \end{tabular}\\ 
  \end{tabular} \\
  \hline
\end{tabular}
\caption{Top 3 recipe retrievals, based on an image query. Ingredients that occur in the query recipe are written in italics. Left: query with matching retrievals; middle: query with some mismatches in main ingredients; right: query with no satisfying retrievals.}
\label{table:retrievals}
\end{table*}
